FAENet: Frame Averaging Equivariant GNN for Materials Modeling

Applications of machine learning techniques for materials modeling typically involve functions known to be equivariant or invariant to specific symmetries. While graph neural networks (GNNs) have proven successful in such tasks, they enforce symmetries via the model architecture, which often reduces their expressivity, scalability and comprehensibility. In this paper, we introduce (1) a flexible framework relying on stochastic frame-averaging (SFA) to make any model E(3)-equivariant or invariant through data transformations. (2) FAENet: a simple, fast and expressive GNN, optimized for SFA, that processes geometric information without any symmetrypreserving design constraints. We prove the validity of our method theoretically and empirically demonstrate its superior accuracy and computational scalability in materials modeling on the OC20 dataset (S2EF, IS2RE) as well as common molecular modeling tasks (QM9, QM7-X). A package implementation is available at https://faenet.readthedocs.io.

==> RANDOM-content.tex <==
\subsection{Motivation}

\textbf{Motivation.} Designing expressive GNNs that are by construction rotation invariant (or equivariant) is essential in many applications, especially for 3D molecular prediction tasks. Nevertheless, for some important instances of symmetries (e.g. $E(3)$), the design of invariant (equivariant) networks is either lacking in expressivity (e.g. \cite{schutt2021equivariant}) or computationally expensive (e.g. \cite{gasteiger2021gemnet}). To avoid this issue, \cite{hu2021forcenet} do not constrain their GNN to satisfy symmetries, allowing more flexible and expressive architectures, and try to equip their GNN with rotation invariance through data augmentation. This line of thinking was confirmed promising by \cite{gerken2022equivariance}. 

\textbf{Contributions.} In this paper, we use a simple yet effective method, called frame averaging \cite{puny2021frame}, to guarantee our GNN rotation invariance or equivariance. The real advantage of this approach is that we can easily design a scalable universal GNN architecture that is not constrained to be rotation invariant, and which can directly use atomic positions in its message passing layers. We therefore propose a the following contributions: 
\begin{enumerate}
    \item A adaptation of frame averaging to bulk gasses, liquids, crystals or mixtures, which involve unit cells and periodic boundary conditions. 
    \item A fast, simple and expressive GNN architecture which directly processes relative information while still preserving data symmetries, as a benefit of frame averaging. 
    \item A thorough evaluation to prove the claims of our GNN, as well as its performance-scalability trade off.
\end{enumerate}



% ----------------



\subsection{Related Work}

Since their introduction as a means to predict quantum chemical properties of small molecules at the density functional theory (DFT) level, GNNs have found many applications in quantum chemistry, drug discovery, CASP, and molecular property prediction. When applied to quantum chemistry tasks, GNNs often use E(3)-invariant 3D information by including radial and angular information. Indeed, these networks leverage the symmetries of the molecules by employing E(3)-SE(3) equivariant convolutions. While SE(3) are computationally expensive due to the use of spherical harmonics, they enable to distinguish between stereoisomers of chiral molecules including enantiomers. E(3)-equivariant models are more scalable and achieve nearly equal perf, but does not enable to distinguish enantiomers (Enantiomers are pairs of compounds with exactly the same connectivity but opposite three-dimensional shapes; i.e mirror images). 


% SchNet \citep{schutt2017schnet} leverages atom distances via a continuous convolution filter to learn a continuous potential energy surface respecting these constraints. Dimenet++ \citep{klicpera2020directional, klicpera2020fast} goes further and includes a directional message passing (MP) mechanism that incorporates bond angles in addition to atom relative distances. However, distances and bond angles do not suffice to uniquely identify the graph 3D structure. This is achieved by SphereNet \citep{liu2021spherical} and GemNet \citep{gasteiger2021gemnet}, which additionally extract torsion information (between quadruplets of nodes). On the downside, these methods are very computationally expensive as they require considering 3-hop neighbourhoods for each update step. Importantly, all these MP methods aim at broad applicability and do not leverage the specific constraints of individual tasks. 

SchNet \cite{schutt2017schnet} is the first E(3)-invariant method which proposes a continuous potential energy surface that respects essential quantum chemical constraints. Their GNN guarantees invariance by using atom distances within continuous convolution filters. Many methods improved over it, such as \cite{unke2019physnet} or Dimenet++ \cite{klicpera2020directional, klicpera2020fast}, which proposed a directional message passing scheme that incorporates bond angles in addition to atom relative distances, processed respectively through spherical harmonics basis and bessel functions. Compared to SchNet, Dimenet++ better captures the overall structure of the 3D graph while remaining E(3)-invariant. However, like the Graphormer model \cite{ying2021transformers} based on Transformers architecture, it does not provide yet a complete representation of the graph 3D structure. Distances and bond angles do not suffice to uniquely identify the graph 3D structure (without using positional info). This has been achieved by SphereNet \cite{liu2021spherical} and GemNet \cite{gasteiger2021gemnet}, which additionally extracted and used torsion information (between quadruplets of nodes) while remaining invariant to symmetries. In particular, GemNet proved that their directional message passing built on spherical representations is a universal approximator for predictions that are invariant to translations, equivariant to permutations and rotations. 
However, these methods are very computationally expensive as they require considering 3-hops neighbourhood to compute torsion angles, for each update step. Even DimeNet++ is expensive given its complex architecture and its edge message passing. \\


TFN \cite{thomas2018tensor} was the first to propose it, building upon Schnet and Harmonics networks for 2D data.  Cormorant \cite{anderson2019cormorant}, SE(3) Transformers \cite{fuchs2020se}, NeuquIP \cite{batzner20223}, SEGNN \cite{brandstetter2021geometric} followed and improved upon TFN, preserving the same general idea. 
Slightly different, PaiNN \cite{schutt2021equivariant} and EGNN \cite{satorras2021n} learn and leverage equivariant embeddings to update the invariant ones, which are also learned and ultimately used to perform the desired tasks. While equivariance is nice theoretical property, broader than invariance and that generalises better to new applications in practice, it is not perfectly adapted to accelerated catalysis, which only requires invariance. Besides, the model is constrained by the equivariant filters based on spherical harmonics and the combination with features through the Clebsch-Gordan tensor product. The required convolution is also very expensive computationally. 

\textbf{Data augmentation}. ForceNet \cite{hu2021forcenet} is interesting because it is neither explicitly invariant nor equivariant. Instead, it simply tries to encourage this property via data augmentation (DA). Although this is not rigorously achieved, as this would be very hard and expensive to enforce properly, it has the benefits of greater model design flexibility and greater scalability since it avoids equivariant convolutions and extracting invariant quantities. 

To avoid this issue, \cite{hu2021forcenet} do not constrain their GNN to satisfy symmetries, allowing more flexible and expressive architectures, and try to equip their GNN with rotation invariance through data augmentation. 

\textbf{Motivation.} Designing expressive GNNs that are by construction rotation invariant (or equivariant) is essential in many applications, especially for 3D molecular prediction tasks. Nevertheless, as evoked, the design of invariant or equivariant networks is either lacking in expressivity (e.g. \cite{schutt2021equivariant}) or computationally expensive (e.g. \cite{gasteiger2021gemnet}). To avoid this issue, \cite{hu2021forcenet} do not constrain their GNN to satisfy symmetries, allowing more flexible and expressive architectures, and try to equip their GNN with rotation invariance through data augmentation. This line of thinking was confirmed promising by \cite{gerken2022equivariance}. The authors showed that data augmentation matched invariant networks for an invariant tasks on 3D images, with much smaller computational cost. However, data augmentation was less desirable for equivariant tasks. Hence, although interesting, using data augmentation based method still lacks theoretical foundations, does not properly respect symmetries and is rather expensive in training. Besides, some studies \cite{esteves2018learning} have shown that aggressive data augmentation like arbitrary 3D rotations on input data will still harm performance. In our work, we would like to capture the best of both worlds: have a fast model whose design is not constrained by symmetries (for maximal expressivity) while enforcing rigorously symmetries to ensure better behaviour and performance. 




% ---------------------------------




\subsection{Terminology}

Geometric prior. An inductive bias incorporating information on the symmetric nature of the system of interest into the neural network architecture. Also known as symmetry prior.

Inductive bias. Set of assumptions that a learning algorithm (e.g., a neural network) uses to learn the target function and to make predictions on previously unseen data points. 

Density Functional Theory (DFT). A quantum mechanical modeling approach used to investigate the electronic structure of molecules. \\

- Rotation. Movement of an object with respect to the radial orientation to a given point.
- Translation. Movement of every point of an object by the same distance in a given direction.
- Reflection. Mapping of an object to itself through a point (inversion), a line or a plane (mirroring). \\


Equivariance. A neural network F applied to an input X is equivariant to a transformation T if the transformation of the input X commutes with the transformation of F(X ), via a transformation T’ of the same symmetry group, such that: $F(T(X))=T'F(X)$. 
NN are therefore equivariant to the actions of a symmetry group on their inputs if and only if each layer of the network “equivalently" transforms under any transformation of that group.

Invariance. Invariance is a special case of equivariance, where F(X ) is invariant to T if T 0 is the trivial group action (i.e., identity): $F(T(X))=T'F(X)=F(X)$

F(X) is neither equivariant nor invariant to T when the transformation of the input X does not commute with the transformation of F(X ):  $F(T(X))\neq T'F(X)$

The concept of equivariance / invariance is transferable to molecular properties, depending on their behaviour when a transformation is applied. 
Example: equilibrium energies, atomic charges, phyisiochemical properties) are invariant to symmetry operations in E(3). 

This is why we would like our NN to be equivariant/invariant to E(3) symmetries. Exceptions would occur if we predict properties that change under these properties (chiral prop). In such case, the inductive bias of equivariant network would not allow the differentiation of symmetry transformed molecules. 

Groups. O(n): ortho group with rotations and reflections. SO(n): rotations only. E(n): euclidean group with rotations relfections translations. SE(n): special euclidean with rotations and translations only. Lie group elements form a differentiable manifold. 


\subsection{Expressivity}

The universality of a GNN is based on its ability to embed two non-isomorphic graphs to distinct points in the target feature space. A model that can distinguish all pairs of nonisomorphic graphs is a universal approximator.
